Pairwise Evaluation of Accent Similarity in Speech Synthesis

Despite growing interest in generating high-fidelity accents, evaluating accent similarity in speech synthesis has been underexplored. We aim to enhance both subjective and objective evaluation methods for accent similarity. Subjectively, we refine the XAB listening test by adding components that achieve higher statistical significance with fewer listeners and lower costs. Our method involves providing listeners with transcriptions, having them highlight perceived accent differences, and implementing meticulous screening for reliability. Objectively, we utilise pronunciation-related metrics, based on distances between vowel formants and phonetic posteriorgrams, to evaluate accent generation. Comparative experiments reveal that these metrics, alongside accent similarity, speaker similarity, and Mel Cepstral Distortion, can be used. Moreover, our findings underscore significant limitations of common metrics like Word Error Rate in assessing underrepresented accents.

==> tabs/literature_review_blv.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.4pt}
\captionsetup{justification=centering}
\caption{Evaluation methods used in various (accent) generation systems/papers. \blue{\underline{Blue}} indicates objective evaluation methods.}
% : No reference speech is provided in these subjective evaluation tests. : These \blue{\underline{CER}} are calculated on non-English languages, such as Mandarin. : Listeners are asked to classify different accent intensity levels rather than different accents in these AID tests.
\label{tab:lit_rev}
\vspace{-1em}
% \tiny
\scriptsize
\renewcommand{\arraystretch}{1}
\begin{tabular}{ll|lllllll}
\toprule
\multicolumn{1}{c}{Category} & \multicolumn{1}{c|}{System/Paper} & \multicolumn{1}{c}{Accent Similarity} & \multicolumn{1}{c}{Speaker Similarity} & \multicolumn{1}{c}{Intelligibility} & \multicolumn{1}{c}{Naturalness} & \multicolumn{1}{c}{Audio Quality} & \multicolumn{1}{c}{F0} & \multicolumn{1}{c}{Duration} \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Zero-Shot\\ TTS\end{tabular}} 
 % & YourTTS, 2022 \cite{casanova2022yourtts} & & XMOS, \blue{\underline{CosSim}} & & MOS & & & \\
 & XTTS, 2024 \cite{casanova2024xtts} & & XMOS, \blue{\underline{CosSim}} & \blue{\underline{CER}} & CMOS, \blue{\underline{UTMOS}} & & & \\
 & VALL-E, 2025 \cite{chen2025neural} & & \blue{\underline{CosSim}} & \blue{\underline{WER}} & CMOS & & & \\
 % & Seed-TTS & & \blue{\underline{CosSim}} & WER, CER & CMOS & & & \\
 & MaskGCT, 2025 \cite{wang2025maskgct} & XMOS, \blue{\underline{CosSim}} & \blue{\underline{CosSim}} & \blue{\underline{WER, CER}} & MOS, CMOS & \blue{\underline{MCD, FSD}} & & \\
 & Zhang et al., 2023 \cite{zhang2023towards} & XMOS(4), \blue{\underline{AID-Acc}} & XMOS(4) & & MOS & & \blue{\underline{RMSE, PCC, DTW}} & \\
 & AccentBox, 2025 \cite{zhong2025accentbox} & XAB, \blue{\underline{CosSim}} & XAB, \blue{\underline{CosSim}} & & AB & & & \\ \midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}Accented\\ TTS\end{tabular}}
 & Zhou et al., 2024 \cite{zhou2024multi} & XAB, XMOS, \blue{\underline{CosSim}} & XAB, XMOS, \blue{\underline{CosSim}} & & AB, MOS & \blue{\underline{MCD}} & \blue{\underline{RMSE, PCC}} & \blue{\underline{FD}} \\
 & Zhou et al., 2024 \cite{zhou2024accented} & XAB, XBWS, \blue{\underline{PPG-KL}} & & & AB, MOS & & \blue{\underline{RMSE, PCC}} & \blue{\underline{FD, RMSE}} \\
 % & Ai-TTS, 2023 \cite{liu2023explicit} &  AID-Acc & & & MOS & & \blue{Moments, DTW} & \\
 & CTA-TTS, 2024 \cite{liu2024controllable} & XMOS,  AID-Acc & & & & MOS, BWS, \blue{\underline{MCD}} & \blue{\underline{Moments, DTW}} & \blue{\underline{MAE}} \\
 % & TTS-MLVAE, 2022 \cite{melechovsky2022learning} & XBWS & XMOS, \blue{EER} & \blue{\underline{WER}} & MOS & \blue{\underline{MCD}} & & \\
 & DART, 2024 \cite{melechovsky2024dart} & XBWS & XBWS, \blue{\underline{CosSim}} & \blue{\underline{WER}} & MOS & \blue{\underline{MCD}} & \blue{\underline{FFE}} & \\
 & RAD-MMM, 2023 \cite{badlani2023rad} & XCMOS, \blue{\underline{CosSim}} & XCMOS & \blue{\underline{CER}} & & & & \\
 % & VANI, 2023 \cite{rohan2023vani} & & XMOS, \blue{\underline{CosSim}} & \blue{\underline{CER}} & MOS & & & \\
 & AccentSpeech, 2022 \cite{zhang2022accentspeech} & XAB & XAB, \blue{\underline{CosSim}} & & AB & & & \blue{\underline{MAE}}  \\
 & Deja et al., 2023 \cite{deja2023diffusion} & MUSHRA,  AID-Acc & XMUSHRA & & MUSHRA & & & \\
 & Yang et al., 2023 \cite{yang2023parameter} & MOS & & \blue{\underline{CER}} & MOS & \blue{\underline{MCD}} & & \\ \midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}Accent\\ Conversion\end{tabular}}
 % & Zhao et al., 2018 \cite{zhao2018accent} & AB & XMOS(15) & & & MOS & & \\
 % & Zhao et al., 2019 \cite{zhao2019foreign} & MOS(9) & XAB & & MOS & MOS & & \\
 & Accentron, 2022 \cite{ding2022accentron} & MOS(9) & XMOS(15) & & & MOS & & \\
 & Quamer et al., 2022 \cite{quamer2022zero} & MOS(9) & XAB & & MOS & & & \\
 & Zhou et al., 2023 \cite{zhou2023tts} & MOS(9) & XMOS(4) & \blue{\underline{WER, PER}} & & MUSHRA & & \\
 & Bai et al., 2024 \cite{bai2024diffusion} & XBWS & XBWS & & MUSHRA & & & \\
 & Chen et al., 2024 \cite{chen2024transfer} & MOS & XAB & \blue{\underline{WER}} & MOS & & & \\
 & Jia et al., 2023 \cite{jia2023zero} & XMOS & XMOS & & MOS & & & \\
 & Jin et al., 2023 \cite{jin2023voice} & XAB & XMOS & & & MOS & & \\
 & Jia et al., 2024 \cite{jia2024convert} & AID-Acc, \blue{\underline{AID-Acc}} & \blue{\underline{CosSim}} & & MOS, \blue{\underline{NISQA}} & & & \\
 & MacST, 2025 \cite{inoue2025macst} & MUSHRA, \blue{\underline{CosSim}} &  \blue{\underline{CosSim}} & \blue{\underline{WER}} & MUSHRA & & & \\ \bottomrule
\end{tabular}
\caption*{\scriptsize{X...: Reference speech is provided for similarity ratings. (\texttt{num}): A \texttt{num}-point rather than 5-point scale is used. \blue{AID-Acc}: accent identification accuracy. \blue{CosSim}: cosine similarity of accent/speaker embeddings. \blue{PPG-KL}: KL divergence of phonetic posteriorgrams. \blue{WER/CER/PER}: word/character/phone error rate. \blue{UTMOS / NISQA}: predicted MOS by \cite{saeki2022utmos} / \cite{mittag2020deep}. \blue{MCD}: mel cepstral distortion. \blue{FSD}: Fréchet speech distance. \blue{RMSE}: root mean square error. \blue{PCC}: Pearson correlation coefficient. \blue{DTW}: DTW alignment cost. \blue{Moments}: see \cite{ren2021fastspeech}. \blue{FFE}: F0 frame error. \blue{FD}: frame difference. \blue{MAE}: mean absolute error.}}
\vspace{-4em}
\end{table*}

==> tabs/obj_corr.tex <==
\begin{figure}[h!]
\centering
\captionsetup{justification=centering}
% \includegraphics[width=1\linewidth, height=1\linewidth, trim = 10 10 160 120, clip]{figs/heatmap_corr_17.pdf}
\includegraphics[width=1\linewidth, height=0.2\linewidth, trim = 85 15 100 10, clip]{figs/heatmap_corr_7_onerow.pdf}
\caption{Spearman Rank Correlation Coefficients (SRCCs) of various objective metrics with hypothesised rank.}
\label{fig:obj_corr}
\end{figure}
